Unveiling Narrative Reasoning Limits of Large Language Models with Trope in Movie Synopses

Large language models (LLMs) equipped with chain-of-thoughts (CoT) prompting have shown significant multi-step reasoning capabilities in factual content like mathematics, commonsense, and logic. However, their performance in narrative reasoning, which demands greater abstraction capabilities, remains unexplored. This study utilizes tropes in movie synopses to assess the abstract reasoning abilities of state-of-the-art LLMs and uncovers their low performance. We introduce a trope-wise querying approach to address these challenges and boost the F1 score by 11.8 points. Moreover, while prior studies suggest that CoT enhances multi-step reasoning, this study shows CoT can cause hallucinations in narrative content, reducing GPT-4's performance. We also introduce an Adversarial Injection method to embed trope-related text tokens into movie synopses without explicit tropes, revealing CoT's heightened sensitivity to such injections. Our comprehensive analysis provides insights for future research directions.

==> data/ChatGPT_CoT_PerTropeF1.tex <==
825
('Big \\"NO!\\"', 2.9)
('Groin Attack', 10.2)
('Meaningful Echo', 10.63)
('Cassandra Truth', 10.64)
('Anti-Hero', 10.72)
('Determinator', 11.21)
('Blatant Lies', 11.52)
('Took a Level in Badass', 11.69)
('Exact Words', 11.76)
('Would Hit a Girl', 12.4)
('Tempting Fate', 12.43)
('Does This Remind You of Anything?', 12.48)
('Only Sane Man', 12.61)
('What the Hell, Hero?', 12.95)
('Earn Your Happy Ending', 13.27)
('Irony', 13.28)
('Crapsack World', 13.31)
("Chekhov's Gunman", 13.47)
('Stealth Pun', 13.54)
('Precision F-Strike', 13.89)
('Hope Spot', 14.32)
("Screw This, I'm Outta Here!", 14.43)
('Laser-Guided Karma', 14.54)
('Faux Affably Evil', 14.72)
('Idiot Ball', 14.77)
('Not So Different', 14.91)
('Batman Gambit', 14.97)
('Smug Snake', 15.13)
('Jerkass Has a Point', 15.13)
('Comically Missing the Point', 15.38)
('Nice Job Breaking It, Hero!', 15.76)
('Disproportionate Retribution', 15.85)
('Red Herring', 15.95)
('Cluster F-Bomb', 16.0)
('Affably Evil', 16.02)
('Hypocritical Humor', 16.14)
('Papa Wolf', 16.57)
("Chekhov's Skill", 16.77)
('Hoist by His Own Petard', 16.89)
('Disappeared Dad', 17.05)
('Karmic Death', 17.2)
('Villainous Breakdown', 17.74)
('The Reveal', 17.94)
('Freudian Excuse', 18.09)
('Curb-Stomp Battle', 18.18)
('My God, What Have I Done?', 18.37)
('Adorkable', 18.44)
('Adult Fear', 18.48)
('Disney Villain Death', 18.71)
('Reasonable Authority Figure', 19.51)
('Fan Disservice', 19.58)
('Black Comedy', 19.6)
('Fanservice', 19.75)
('Ironic Echo', 19.81)
('Heroic BSoD', 19.84)
('Police are Useless', 20.39)
('Abusive Parents', 20.72)
('Even Evil Has Standards', 20.96)
('Roaring Rampage of Revenge', 21.11)
('Big Damn Heroes', 21.14)
('Would Hurt a Child', 21.5)
('Gory Discretion Shot', 22.54)
('Pet the Dog', 22.7)
('Heel Face Turn', 22.91)
('Body Horror', 22.99)
('Badass Boast', 23.24)
('Brick Joke', 23.79)
('Ms. Fanservice', 23.81)
('Berserk Button', 24.07)
('Kick the Dog', 24.26)
('\\"The Reason You Suck\\" Speech', 24.86)
('Too Dumb to Live', 25.0)
('Jerk with a Heart of Gold', 25.23)
('Butt-Monkey', 25.58)
('The Dragon', 25.88)
('Karma Houdini', 26.49)
('Asshole Victim', 27.71)
('Jerkass', 28.27)
('Bittersweet Ending', 29.46)
('Heroic Sacrifice', 31.88)
('Action Girl', 32.26)
('Off with His Head!', 32.38)
('Deadpan Snarker', 34.01)
('Impaled with Extreme Prejudice', 34.21)
('The Alcoholic', 34.92)
('Your Cheating Heart', 35.02)
('Oh, Crap!', 37.02)
('Foreshadowing', 37.1)
('Cool Car', 37.61)
('Ax-Crazy', 37.63)
('Downer Ending', 38.05)
("Chekhov's Gun", 40.0)
('Big Bad', 42.81)
('Driven to Suicide', 47.89)
('Eye Scream', 50.67)


==> data/ChatGPT_CoT_PerTropePrecision.tex <==
('Meaningful Echo', 5.63)
('Anti-Hero', 5.66)
('Cassandra Truth', 5.68)
('Determinator', 5.96)
('Took a Level in Badass', 6.27)
('Exact Words', 6.29)
('Tempting Fate', 6.63)
('Blatant Lies', 6.63)
('Does This Remind You of Anything?', 6.83)
('What the Hell, Hero?', 7.02)
('Would Hit a Girl', 7.08)
('Only Sane Man', 7.09)
('Earn Your Happy Ending', 7.11)
('Irony', 7.16)
('Crapsack World', 7.18)
("Chekhov's Gunman", 7.6)
('Big \\"NO!\\"', 7.69)
('Hope Spot', 7.73)
('Laser-Guided Karma', 7.86)
('Faux Affably Evil', 7.97)
('Not So Different', 8.08)
('Smug Snake', 8.2)
('Batman Gambit', 8.23)
('Jerkass Has a Point', 8.26)
("Screw This, I'm Outta Here!", 8.27)
('Comically Missing the Point', 8.44)
('Nice Job Breaking It, Hero!', 8.57)
('Disproportionate Retribution', 8.61)
('Stealth Pun', 8.72)
('Affably Evil', 8.75)
('Red Herring', 8.78)
('Hypocritical Humor', 8.79)
("Chekhov's Skill", 9.22)
('Hoist by His Own Petard', 9.25)
('Papa Wolf', 9.26)
('Idiot Ball', 9.36)
('Karmic Death', 9.49)
('Villainous Breakdown', 9.93)
('The Reveal', 10.08)
('Disappeared Dad', 10.23)
('Adult Fear', 10.24)
('My God, What Have I Done?', 10.43)
('Curb-Stomp Battle', 10.47)
('Ironic Echo', 11.02)
('Adorkable', 11.16)
('Black Comedy', 11.27)
('Heroic BSoD', 11.41)
('Reasonable Authority Figure', 11.55)
('Police are Useless', 11.69)
('Abusive Parents', 11.81)
('Freudian Excuse', 11.84)
('Even Evil Has Standards', 11.98)
('Disney Villain Death', 12.04)
('Big Damn Heroes', 12.05)
('Roaring Rampage of Revenge', 12.08)
('Fan Disservice', 12.28)
('Would Hurt a Child', 12.64)
('Gory Discretion Shot', 13.51)
('Precision F-Strike', 13.7)
('Heel Face Turn', 13.8)
('Body Horror', 13.82)
('Jerk with a Heart of Gold', 14.72)
('Brick Joke', 14.75)
('Berserk Button', 14.84)
('Badass Boast', 15.3)
('Pet the Dog', 16.0)
('Too Dumb to Live', 16.11)
('Butt-Monkey', 16.12)
('Asshole Victim', 16.37)
('Jerkass', 16.88)
('Bittersweet Ending', 17.34)
('Kick the Dog', 17.45)
('Karma Houdini', 17.89)
('The Dragon', 18.33)
('Fanservice', 19.05)
('\\"The Reason You Suck\\" Speech', 19.83)
('Heroic Sacrifice', 21.15)
('Deadpan Snarker', 21.83)
('Oh, Crap!', 22.77)
('Foreshadowing', 22.83)
('Action Girl', 22.94)
('The Alcoholic', 23.24)
('Impaled with Extreme Prejudice', 23.85)
('Downer Ending', 24.02)
('Ms. Fanservice', 24.19)
('Your Cheating Heart', 25.0)
('Off with His Head!', 25.37)
('Ax-Crazy', 25.96)
("Chekhov's Gun", 27.74)
('Cluster F-Bomb', 28.57)
('Cool Car', 28.57)
('Groin Attack', 31.25)
('Driven to Suicide', 35.92)
('Big Bad', 37.84)
('Eye Scream', 47.5)


==> data/ChatGPT_CoT_PerTropeRecall.tex <==
('Big \\"NO!\\"', 1.79)
('Groin Attack', 6.1)
('Cluster F-Bomb', 11.11)
('Precision F-Strike', 14.08)
('Fanservice', 20.51)
('Ms. Fanservice', 23.44)
('Stealth Pun', 30.23)
('\\"The Reason You Suck\\" Speech', 33.33)
('Idiot Ball', 34.92)
('Freudian Excuse', 38.3)
('Pet the Dog', 39.02)
('Kick the Dog', 39.78)
('Disney Villain Death', 41.94)
('The Dragon', 44.0)
('Blatant Lies', 44.0)
('Off with His Head!', 44.74)
('Badass Boast', 48.28)
('Fan Disservice', 48.28)
('Big Bad', 49.3)
('Would Hit a Girl', 50.0)
('Karma Houdini', 51.0)
('Disappeared Dad', 51.16)
('Adorkable', 53.06)
('Eye Scream', 54.29)
('Action Girl', 54.35)
('Cool Car', 55.0)
('Too Dumb to Live', 55.79)
("Screw This, I'm Outta Here!", 56.45)
('Only Sane Man', 57.14)
('Your Cheating Heart', 58.46)
("Chekhov's Gunman", 59.09)
('Impaled with Extreme Prejudice', 60.47)
('Brick Joke', 61.46)
('Butt-Monkey', 61.97)
('Reasonable Authority Figure', 62.75)
('Berserk Button', 63.73)
('Heroic Sacrifice', 64.71)
('Heel Face Turn', 67.21)
('Gory Discretion Shot', 67.8)
('Body Horror', 68.18)
('Ax-Crazy', 68.35)
('Curb-Stomp Battle', 68.89)
('The Alcoholic', 70.21)
("Chekhov's Gun", 71.66)
('Would Hurt a Child', 71.74)
('Driven to Suicide', 71.83)
('Does This Remind You of Anything?', 72.41)
('Black Comedy', 75.0)
('Heroic BSoD', 76.12)
('My God, What Have I Done?', 76.81)
('Deadpan Snarker', 76.97)
('Papa Wolf', 78.95)
('Police are Useless', 79.66)
('The Reveal', 81.54)
('Batman Gambit', 82.5)
('Villainous Breakdown', 83.02)
('Roaring Rampage of Revenge', 83.33)
('What the Hell, Hero?', 83.33)
('Even Evil Has Standards', 83.56)
('Cassandra Truth', 83.72)
('Abusive Parents', 84.31)
('Big Damn Heroes', 85.71)
('Took a Level in Badass', 85.71)
('Comically Missing the Point', 86.67)
('Red Herring', 86.67)
('Jerkass', 86.89)
('Jerk with a Heart of Gold', 88.3)
('Jerkass Has a Point', 90.0)
('Exact Words', 90.0)
('Asshole Victim', 90.2)
('Irony', 90.91)
('Crapsack World', 91.11)
('Downer Ending', 91.49)
('Karmic Death', 91.49)
("Chekhov's Skill", 92.98)
('Determinator', 93.75)
('Affably Evil', 94.55)
('Adult Fear', 94.87)
('Meaningful Echo', 95.0)
('Faux Affably Evil', 96.36)
('Laser-Guided Karma', 96.43)
('Hope Spot', 96.72)
('Not So Different', 96.83)
('Hoist by His Own Petard', 96.97)
('Ironic Echo', 97.67)
('Bittersweet Ending', 97.87)
('Tempting Fate', 98.15)
('Earn Your Happy Ending', 98.15)
('Smug Snake', 98.21)
('Hypocritical Humor', 98.33)
('Nice Job Breaking It, Hero!', 98.53)
('Oh, Crap!', 98.86)
('Foreshadowing', 98.9)
('Anti-Hero', 100.0)
('Disproportionate Retribution', 100.0)


==> data/ChatGPT_base_PerTropeF1.tex <==
('Too Dumb to Live', 0.0)
('Disney Villain Death', 0.0)
('Precision F-Strike', 0.0)
('Groin Attack', 2.35)
('Stealth Pun', 3.28)
('Asshole Victim', 3.81)
("Screw This, I'm Outta Here!", 4.49)
('Blatant Lies', 4.82)
('Cluster F-Bomb', 4.88)
('Exact Words', 5.56)
('Fan Disservice', 6.45)
('Karma Houdini', 6.84)
('Would Hit a Girl', 6.9)
('\\"The Reason You Suck\\" Speech', 7.23)
('Freudian Excuse', 7.79)
('Gory Discretion Shot', 8.11)
('Red Herring', 8.7)
('Does This Remind You of Anything?', 9.09)
('What the Hell, Hero?', 9.09)
('Irony', 9.61)
('Kick the Dog', 9.76)
('Off with His Head!', 10.34)
('Only Sane Man', 11.76)
("Chekhov's Gunman", 11.76)
('Would Hurt a Child', 12.31)
('Tempting Fate', 12.33)
('Meaningful Echo', 12.33)
('Idiot Ball', 13.08)
('Disproportionate Retribution', 13.22)
('Ms. Fanservice', 13.48)
('Big Bad', 13.75)
('Hypocritical Humor', 13.79)
('Faux Affably Evil', 13.95)
('Batman Gambit', 14.49)
("Chekhov's Skill", 14.67)
('My God, What Have I Done?', 14.97)
('Butt-Monkey', 15.38)
('Jerkass', 15.48)
('Fanservice', 15.56)
('Cassandra Truth', 15.65)
('Determinator', 15.73)
('Brick Joke', 15.75)
('Not So Different', 16.3)
('Laser-Guided Karma', 16.97)
('Adorkable', 17.02)
('Badass Boast', 17.07)
('Big \\"NO!\\"', 17.39)
('Hoist by His Own Petard', 17.71)
('Jerkass Has a Point', 17.78)
('Even Evil Has Standards', 17.89)
('Downer Ending', 17.91)
('Curb-Stomp Battle', 18.64)
('Affably Evil', 18.71)
('Ironic Echo', 19.15)
('The Reveal', 19.53)
('Deadpan Snarker', 19.64)
('Disappeared Dad', 19.64)
('Heroic BSoD', 19.69)
('Smug Snake', 19.82)
('Took a Level in Badass', 19.86)
('Karmic Death', 20.21)
('Pet the Dog', 20.45)
('Heel Face Turn', 20.69)
('Villainous Breakdown', 20.78)
('Reasonable Authority Figure', 20.81)
('Roaring Rampage of Revenge', 21.05)
('Crapsack World', 21.85)
('Anti-Hero', 22.01)
('Earn Your Happy Ending', 22.34)
('Berserk Button', 22.46)
('Big Damn Heroes', 22.58)
('Comically Missing the Point', 22.73)
('Nice Job Breaking It, Hero!', 22.9)
('Police are Useless', 23.36)
('Hope Spot', 23.46)
('Adult Fear', 25.0)
('Your Cheating Heart', 25.0)
('Black Comedy', 25.93)
('Body Horror', 26.57)
('Ax-Crazy', 26.82)
('Impaled with Extreme Prejudice', 27.78)
('Papa Wolf', 28.17)
('The Dragon', 28.32)
('Heroic Sacrifice', 28.44)
('Action Girl', 28.8)
('Jerk with a Heart of Gold', 31.05)
('Bittersweet Ending', 34.57)
("Chekhov's Gun", 35.7)
('Oh, Crap!', 35.95)
('Foreshadowing', 37.34)
('Abusive Parents', 38.02)
('Eye Scream', 38.38)
('Cool Car', 39.13)
('Driven to Suicide', 42.65)
('The Alcoholic', 44.68)


==> data/ChatGPT_base_PerTropePrecision.tex <==
('Too Dumb to Live', 0.0)
('Disney Villain Death', 0.0)
('Precision F-Strike', 0.0)
('Stealth Pun', 5.56)
('Blatant Lies', 6.06)
('Exact Words', 6.25)
('Irony', 6.32)
("Screw This, I'm Outta Here!", 7.41)
('Would Hit a Girl', 7.69)
('What the Hell, Hero?', 7.69)
('Meaningful Echo', 8.49)
('Red Herring', 8.51)
("Chekhov's Gunman", 8.7)
('Determinator', 8.82)
('Tempting Fate', 9.78)
('Only Sane Man', 10.0)
('Freudian Excuse', 10.0)
('Kick the Dog', 11.27)
("Chekhov's Skill", 11.83)
('Cassandra Truth', 12.5)
('Laser-Guided Karma', 12.84)
('Anti-Hero', 13.22)
('Roaring Rampage of Revenge', 13.33)
('Villainous Breakdown', 13.48)
('Karmic Death', 13.48)
('Hoist by His Own Petard', 13.49)
('Reasonable Authority Figure', 13.53)
('Fanservice', 13.73)
('The Reveal', 14.0)
('My God, What Have I Done?', 14.1)
('Took a Level in Badass', 14.14)
('Disproportionate Retribution', 14.29)
('Off with His Head!', 15.0)
('Curb-Stomp Battle', 15.07)
('Heroic BSoD', 15.08)
('Big Damn Heroes', 15.14)
('Not So Different', 15.28)
('Affably Evil', 15.48)
('Earn Your Happy Ending', 15.67)
('Idiot Ball', 15.91)
('Disappeared Dad', 15.94)
('Batman Gambit', 17.24)
('Crapsack World', 17.57)
('Ironic Echo', 17.65)
('Adult Fear', 17.74)
('Adorkable', 17.78)
('Hope Spot', 17.8)
('Pet the Dog', 19.15)
('Body Horror', 19.19)
('Faux Affably Evil', 19.35)
('Smug Snake', 20.0)
('Gory Discretion Shot', 20.0)
('Cluster F-Bomb', 20.0)
('Heroic Sacrifice', 20.38)
('Police are Useless', 20.51)
('Would Hurt a Child', 21.05)
('\\"The Reason You Suck\\" Speech', 21.43)
('Heel Face Turn', 21.82)
('Even Evil Has Standards', 22.0)
('Big \\"NO!\\"', 22.22)
('Hypocritical Humor', 22.22)
('Action Girl', 22.78)
('Comically Missing the Point', 23.26)
('Karma Houdini', 23.53)
('Nice Job Breaking It, Hero!', 23.81)
('Ax-Crazy', 24.0)
('Ms. Fanservice', 24.0)
('Butt-Monkey', 24.24)
('Berserk Button', 24.71)
('Black Comedy', 25.0)
('The Dragon', 25.4)
('Jerkass Has a Point', 26.67)
('Oh, Crap!', 27.09)
('Jerk with a Heart of Gold', 27.2)
('Jerkass', 28.26)
('Badass Boast', 29.17)
('Downer Ending', 30.0)
('Papa Wolf', 30.3)
('Foreshadowing', 30.53)
('Deadpan Snarker', 30.56)
('Bittersweet Ending', 30.6)
("Chekhov's Gun", 31.2)
('Brick Joke', 32.26)
('Abusive Parents', 32.86)
('Your Cheating Heart', 33.33)
('Groin Attack', 33.33)
('Impaled with Extreme Prejudice', 34.48)
('Cool Car', 34.62)
('Does This Remind You of Anything?', 37.5)
('Driven to Suicide', 44.62)
('The Alcoholic', 44.68)
('Fan Disservice', 50.0)
('Big Bad', 61.11)
('Eye Scream', 65.52)
('Asshole Victim', 66.67)


==> data/ChatGPT_base_PerTropeRecall.tex <==
('Too Dumb to Live', 0.0)
('Disney Villain Death', 0.0)
('Precision F-Strike', 0.0)
('Groin Attack', 1.22)
('Asshole Victim', 1.96)
('Stealth Pun', 2.33)
('Cluster F-Bomb', 2.78)
("Screw This, I'm Outta Here!", 3.23)
('Fan Disservice', 3.45)
('Blatant Lies', 4.0)
('Karma Houdini', 4.0)
('\\"The Reason You Suck\\" Speech', 4.35)
('Exact Words', 5.0)
('Gory Discretion Shot', 5.08)
('Does This Remind You of Anything?', 5.17)
('Would Hit a Girl', 6.25)
('Freudian Excuse', 6.38)
('Big Bad', 7.75)
('Off with His Head!', 7.89)
('Kick the Dog', 8.6)
('Would Hurt a Child', 8.7)
('Red Herring', 8.89)
('Ms. Fanservice', 9.38)
('Hypocritical Humor', 10.0)
('Brick Joke', 10.42)
('Jerkass', 10.66)
('Faux Affably Evil', 10.91)
('Idiot Ball', 11.11)
('What the Hell, Hero?', 11.11)
('Butt-Monkey', 11.27)
('Badass Boast', 12.07)
('Disproportionate Retribution', 12.31)
('Batman Gambit', 12.5)
('Downer Ending', 12.77)
('Jerkass Has a Point', 13.33)
('Only Sane Man', 14.29)
('Big \\"NO!\\"', 14.29)
('Deadpan Snarker', 14.47)
('Even Evil Has Standards', 15.07)
('My God, What Have I Done?', 15.94)
('Adorkable', 16.33)
('Tempting Fate', 16.67)
('Not So Different', 17.46)
('Fanservice', 17.95)
("Chekhov's Gunman", 18.18)
("Chekhov's Skill", 19.3)
('Smug Snake', 19.64)
('Heel Face Turn', 19.67)
('Your Cheating Heart', 20.0)
('Irony', 20.0)
('Berserk Button', 20.59)
('Cassandra Truth', 20.93)
('Ironic Echo', 20.93)
('Pet the Dog', 21.95)
('Nice Job Breaking It, Hero!', 22.06)
('Comically Missing the Point', 22.22)
('Meaningful Echo', 22.5)
('Impaled with Extreme Prejudice', 23.26)
('Affably Evil', 23.64)
('Curb-Stomp Battle', 24.44)
('Laser-Guided Karma', 25.0)
('Disappeared Dad', 25.58)
('Hoist by His Own Petard', 25.76)
('Papa Wolf', 26.32)
('Black Comedy', 26.92)
('Police are Useless', 27.12)
('Eye Scream', 27.14)
('Heroic BSoD', 28.36)
('Crapsack World', 28.89)
('Ax-Crazy', 30.38)
('The Dragon', 32.0)
('The Reveal', 32.31)
('Took a Level in Badass', 33.33)
('Hope Spot', 34.43)
('Jerk with a Heart of Gold', 36.17)
('Earn Your Happy Ending', 38.89)
('Action Girl', 39.13)
('Bittersweet Ending', 39.72)
('Karmic Death', 40.43)
('Driven to Suicide', 40.85)
("Chekhov's Gun", 41.71)
('Adult Fear', 42.31)
('Body Horror', 43.18)
('Big Damn Heroes', 44.44)
('The Alcoholic', 44.68)
('Cool Car', 45.0)
('Abusive Parents', 45.1)
('Reasonable Authority Figure', 45.1)
('Villainous Breakdown', 45.28)
('Heroic Sacrifice', 47.06)
('Foreshadowing', 48.07)
('Roaring Rampage of Revenge', 50.0)
('Oh, Crap!', 53.41)
('Anti-Hero', 65.71)
('Determinator', 72.92)


==> data/Delta_ChatGPTCot_ChatGPTBase.tex <==
Big Bad: Delta: 29.06. GPT3_CoT: 42.81 GPT3_base: 13.75
Too Dumb to Live: Delta: 25.0. GPT3_CoT: 25.0 GPT3_base: 0.0
Asshole Victim: Delta: 23.9. GPT3_CoT: 27.71 GPT3_base: 3.81
Off with His Head!: Delta: 22.04. GPT3_CoT: 32.38 GPT3_base: 10.34
Downer Ending: Delta: 20.14. GPT3_CoT: 38.05 GPT3_base: 17.91
Karma Houdini: Delta: 19.65. GPT3_CoT: 26.49 GPT3_base: 6.84
Disney Villain Death: Delta: 18.71. GPT3_CoT: 18.71 GPT3_base: 0.0
 "The Reason You Suck" Speech: Delta: 17.63. GPT3_CoT: 24.86 GPT3_base: 7.23
Kick the Dog: Delta: 14.5. GPT3_CoT: 24.26 GPT3_base: 9.76
Gory Discretion Shot: Delta: 14.43. GPT3_CoT: 22.54 GPT3_base: 8.11
Deadpan Snarker: Delta: 14.37. GPT3_CoT: 34.01 GPT3_base: 19.64
Precision F-Strike: Delta: 13.89. GPT3_CoT: 13.89 GPT3_base: 0.0
Fan Disservice: Delta: 13.13. GPT3_CoT: 19.58 GPT3_base: 6.45
Jerkass: Delta: 12.79. GPT3_CoT: 28.27 GPT3_base: 15.48
Eye Scream: Delta: 12.29. GPT3_CoT: 50.67 GPT3_base: 38.38
Cluster F-Bomb: Delta: 11.12. GPT3_CoT: 16.0 GPT3_base: 4.88
Ax-Crazy: Delta: 10.81. GPT3_CoT: 37.63 GPT3_base: 26.82
Ms. Fanservice: Delta: 10.33. GPT3_CoT: 23.81 GPT3_base: 13.48
Freudian Excuse: Delta: 10.3. GPT3_CoT: 18.09 GPT3_base: 7.79
Stealth Pun: Delta: 10.26. GPT3_CoT: 13.54 GPT3_base: 3.28
Butt-Monkey: Delta: 10.2. GPT3_CoT: 25.58 GPT3_base: 15.38
Your Cheating Heart: Delta: 10.02. GPT3_CoT: 35.02 GPT3_base: 25.0
Screw This, I'm Outta Here!: Delta: 9.94. GPT3_CoT: 14.43 GPT3_base: 4.49
Would Hurt a Child: Delta: 9.19. GPT3_CoT: 21.5 GPT3_base: 12.31
Brick Joke: Delta: 8.04. GPT3_CoT: 23.79 GPT3_base: 15.75
Groin Attack: Delta: 7.85. GPT3_CoT: 10.2 GPT3_base: 2.35
Red Herring: Delta: 7.25. GPT3_CoT: 15.95 GPT3_base: 8.7
Blatant Lies: Delta: 6.7. GPT3_CoT: 11.52 GPT3_base: 4.82
Impaled with Extreme Prejudice: Delta: 6.43. GPT3_CoT: 34.21 GPT3_base: 27.78
Exact Words: Delta: 6.2. GPT3_CoT: 11.76 GPT3_base: 5.56
Badass Boast: Delta: 6.17. GPT3_CoT: 23.24 GPT3_base: 17.07
Would Hit a Girl: Delta: 5.5. GPT3_CoT: 12.4 GPT3_base: 6.9
Driven to Suicide: Delta: 5.24. GPT3_CoT: 47.89 GPT3_base: 42.65
Chekhov's Gun: Delta: 4.3. GPT3_CoT: 40.0 GPT3_base: 35.7
Fanservice: Delta: 4.19. GPT3_CoT: 19.75 GPT3_base: 15.56
What the Hell, Hero?: Delta: 3.86. GPT3_CoT: 12.95 GPT3_base: 9.09
Irony: Delta: 3.67. GPT3_CoT: 13.28 GPT3_base: 9.61
Action Girl: Delta: 3.46. GPT3_CoT: 32.26 GPT3_base: 28.8
Heroic Sacrifice: Delta: 3.44. GPT3_CoT: 31.88 GPT3_base: 28.44
My God, What Have I Done?: Delta: 3.4. GPT3_CoT: 18.37 GPT3_base: 14.97
Does This Remind You of Anything?: Delta: 3.39. GPT3_CoT: 12.48 GPT3_base: 9.09
Even Evil Has Standards: Delta: 3.07. GPT3_CoT: 20.96 GPT3_base: 17.89
Disproportionate Retribution: Delta: 2.63. GPT3_CoT: 15.85 GPT3_base: 13.22
Hypocritical Humor: Delta: 2.35. GPT3_CoT: 16.14 GPT3_base: 13.79
Pet the Dog: Delta: 2.25. GPT3_CoT: 22.7 GPT3_base: 20.45
Heel Face Turn: Delta: 2.22. GPT3_CoT: 22.91 GPT3_base: 20.69
Chekhov's Skill: Delta: 2.1. GPT3_CoT: 16.77 GPT3_base: 14.67
Chekhov's Gunman: Delta: 1.71. GPT3_CoT: 13.47 GPT3_base: 11.76
Idiot Ball: Delta: 1.69. GPT3_CoT: 14.77 GPT3_base: 13.08
Berserk Button: Delta: 1.61. GPT3_CoT: 24.07 GPT3_base: 22.46
Adorkable: Delta: 1.42. GPT3_CoT: 18.44 GPT3_base: 17.02
Oh, Crap!: Delta: 1.07. GPT3_CoT: 37.02 GPT3_base: 35.95
Only Sane Man: Delta: 0.85. GPT3_CoT: 12.61 GPT3_base: 11.76
Faux Affably Evil: Delta: 0.77. GPT3_CoT: 14.72 GPT3_base: 13.95
Ironic Echo: Delta: 0.66. GPT3_CoT: 19.81 GPT3_base: 19.15
Batman Gambit: Delta: 0.48. GPT3_CoT: 14.97 GPT3_base: 14.49
Heroic BSoD: Delta: 0.15. GPT3_CoT: 19.84 GPT3_base: 19.69
Tempting Fate: Delta: 0.1. GPT3_CoT: 12.43 GPT3_base: 12.33
Roaring Rampage of Revenge: Delta: 0.06. GPT3_CoT: 21.11 GPT3_base: 21.05
Foreshadowing: Delta: -0.24. GPT3_CoT: 37.1 GPT3_base: 37.34
Curb-Stomp Battle: Delta: -0.46. GPT3_CoT: 18.18 GPT3_base: 18.64
Hoist by His Own Petard: Delta: -0.82. GPT3_CoT: 16.89 GPT3_base: 17.71
Reasonable Authority Figure: Delta: -1.3. GPT3_CoT: 19.51 GPT3_base: 20.81
Not So Different: Delta: -1.39. GPT3_CoT: 14.91 GPT3_base: 16.3
Big Damn Heroes: Delta: -1.44. GPT3_CoT: 21.14 GPT3_base: 22.58
Cool Car: Delta: -1.52. GPT3_CoT: 37.61 GPT3_base: 39.13
The Reveal: Delta: -1.59. GPT3_CoT: 17.94 GPT3_base: 19.53
Meaningful Echo: Delta: -1.7. GPT3_CoT: 10.63 GPT3_base: 12.33
Laser-Guided Karma: Delta: -2.43. GPT3_CoT: 14.54 GPT3_base: 16.97
The Dragon: Delta: -2.44. GPT3_CoT: 25.88 GPT3_base: 28.32
Disappeared Dad: Delta: -2.59. GPT3_CoT: 17.05 GPT3_base: 19.64
Jerkass Has a Point: Delta: -2.65. GPT3_CoT: 15.13 GPT3_base: 17.78
Affably Evil: Delta: -2.69. GPT3_CoT: 16.02 GPT3_base: 18.71
Police are Useless: Delta: -2.97. GPT3_CoT: 20.39 GPT3_base: 23.36
Karmic Death: Delta: -3.01. GPT3_CoT: 17.2 GPT3_base: 20.21
Villainous Breakdown: Delta: -3.04. GPT3_CoT: 17.74 GPT3_base: 20.78
Body Horror: Delta: -3.58. GPT3_CoT: 22.99 GPT3_base: 26.57
Determinator: Delta: -4.52. GPT3_CoT: 11.21 GPT3_base: 15.73
Smug Snake: Delta: -4.69. GPT3_CoT: 15.13 GPT3_base: 19.82
Cassandra Truth: Delta: -5.01. GPT3_CoT: 10.64 GPT3_base: 15.65
Bittersweet Ending: Delta: -5.11. GPT3_CoT: 29.46 GPT3_base: 34.57
Jerk with a Heart of Gold: Delta: -5.82. GPT3_CoT: 25.23 GPT3_base: 31.05
Black Comedy: Delta: -6.33. GPT3_CoT: 19.6 GPT3_base: 25.93
Adult Fear: Delta: -6.52. GPT3_CoT: 18.48 GPT3_base: 25.0
Nice Job Breaking It, Hero!: Delta: -7.14. GPT3_CoT: 15.76 GPT3_base: 22.9
Comically Missing the Point: Delta: -7.35. GPT3_CoT: 15.38 GPT3_base: 22.73
Took a Level in Badass: Delta: -8.17. GPT3_CoT: 11.69 GPT3_base: 19.86
Crapsack World: Delta: -8.54. GPT3_CoT: 13.31 GPT3_base: 21.85
Earn Your Happy Ending: Delta: -9.07. GPT3_CoT: 13.27 GPT3_base: 22.34
Hope Spot: Delta: -9.14. GPT3_CoT: 14.32 GPT3_base: 23.46
The Alcoholic: Delta: -9.76. GPT3_CoT: 34.92 GPT3_base: 44.68
Anti-Hero: Delta: -11.29. GPT3_CoT: 10.72 GPT3_base: 22.01
Papa Wolf: Delta: -11.6. GPT3_CoT: 16.57 GPT3_base: 28.17
Big "NO!": Delta: -14.49. GPT3_CoT: 2.9 GPT3_base: 17.39
Abusive Parents: Delta: -17.3. GPT3_CoT: 20.72 GPT3_base: 38.02
1
​

==> data/Delta_GPT4base_ChatGPTbase.tex <==
Disney Villain Death: Delta: 40.96. GPT4_base: 40.96 GPT3_base: 0.0
Downer Ending: Delta: 37.53. GPT4_base: 55.44 GPT3_base: 17.91
Off with His Head!: Delta: 36.17. GPT4_base: 46.51 GPT3_base: 10.34
Asshole Victim: Delta: 33.8. GPT4_base: 37.61 GPT3_base: 3.81
Too Dumb to Live: Delta: 31.47. GPT4_base: 31.47 GPT3_base: 0.0
Karma Houdini: Delta: 25.32. GPT4_base: 32.16 GPT3_base: 6.84
 "The Reason You Suck" Speech: Delta: 24.67. GPT4_base: 31.9 GPT3_base: 7.23
Big Bad: Delta: 24.25. GPT4_base: 38.0 GPT3_base: 13.75
Red Herring: Delta: 23.21. GPT4_base: 31.91 GPT3_base: 8.7
Fan Disservice: Delta: 22.91. GPT4_base: 29.36 GPT3_base: 6.45
Kick the Dog: Delta: 20.71. GPT4_base: 30.47 GPT3_base: 9.76
Jerkass: Delta: 18.34. GPT4_base: 33.82 GPT3_base: 15.48
Batman Gambit: Delta: 17.77. GPT4_base: 32.26 GPT3_base: 14.49
Cluster F-Bomb: Delta: 17.34. GPT4_base: 22.22 GPT3_base: 4.88
Screw This, I'm Outta Here!: Delta: 16.52. GPT4_base: 21.01 GPT3_base: 4.49
Gory Discretion Shot: Delta: 16.42. GPT4_base: 24.53 GPT3_base: 8.11
Would Hurt a Child: Delta: 16.26. GPT4_base: 28.57 GPT3_base: 12.31
Roaring Rampage of Revenge: Delta: 16.22. GPT4_base: 37.27 GPT3_base: 21.05
Impaled with Extreme Prejudice: Delta: 14.64. GPT4_base: 42.42 GPT3_base: 27.78
Adorkable: Delta: 14.23. GPT4_base: 31.25 GPT3_base: 17.02
Groin Attack: Delta: 13.65. GPT4_base: 16.0 GPT3_base: 2.35
Smug Snake: Delta: 13.51. GPT4_base: 33.33 GPT3_base: 19.82
Disproportionate Retribution: Delta: 13.12. GPT4_base: 26.34 GPT3_base: 13.22
Faux Affably Evil: Delta: 13.08. GPT4_base: 27.03 GPT3_base: 13.95
Curb-Stomp Battle: Delta: 12.94. GPT4_base: 31.58 GPT3_base: 18.64
Butt-Monkey: Delta: 12.87. GPT4_base: 28.25 GPT3_base: 15.38
Ax-Crazy: Delta: 12.7. GPT4_base: 39.52 GPT3_base: 26.82
Heel Face Turn: Delta: 12.64. GPT4_base: 33.33 GPT3_base: 20.69
Only Sane Man: Delta: 11.77. GPT4_base: 23.53 GPT3_base: 11.76
Blatant Lies: Delta: 11.37. GPT4_base: 16.19 GPT3_base: 4.82
Chekhov's Skill: Delta: 11.21. GPT4_base: 25.88 GPT3_base: 14.67
Hoist by His Own Petard: Delta: 11.09. GPT4_base: 28.8 GPT3_base: 17.71
Your Cheating Heart: Delta: 10.96. GPT4_base: 35.96 GPT3_base: 25.0
What the Hell, Hero?: Delta: 10.14. GPT4_base: 19.23 GPT3_base: 9.09
Ms. Fanservice: Delta: 9.96. GPT4_base: 23.44 GPT3_base: 13.48
Hope Spot: Delta: 9.63. GPT4_base: 33.09 GPT3_base: 23.46
Affably Evil: Delta: 9.61. GPT4_base: 28.32 GPT3_base: 18.71
Villainous Breakdown: Delta: 9.22. GPT4_base: 30.0 GPT3_base: 20.78
Heroic Sacrifice: Delta: 9.18. GPT4_base: 37.62 GPT3_base: 28.44
My God, What Have I Done?: Delta: 9.1. GPT4_base: 24.07 GPT3_base: 14.97
Would Hit a Girl: Delta: 8.37. GPT4_base: 15.27 GPT3_base: 6.9
Precision F-Strike: Delta: 8.33. GPT4_base: 8.33 GPT3_base: 0.0
Heroic BSoD: Delta: 8.18. GPT4_base: 27.87 GPT3_base: 19.69
Badass Boast: Delta: 7.93. GPT4_base: 25.0 GPT3_base: 17.07
Freudian Excuse: Delta: 7.9. GPT4_base: 15.69 GPT3_base: 7.79
Abusive Parents: Delta: 7.43. GPT4_base: 45.45 GPT3_base: 38.02
Irony: Delta: 7.42. GPT4_base: 17.03 GPT3_base: 9.61
Eye Scream: Delta: 7.07. GPT4_base: 45.45 GPT3_base: 38.38
Not So Different: Delta: 6.87. GPT4_base: 23.17 GPT3_base: 16.3
Berserk Button: Delta: 6.0. GPT4_base: 28.46 GPT3_base: 22.46
Tempting Fate: Delta: 5.74. GPT4_base: 18.07 GPT3_base: 12.33
Oh, Crap!: Delta: 5.4. GPT4_base: 41.35 GPT3_base: 35.95
Even Evil Has Standards: Delta: 5.32. GPT4_base: 23.21 GPT3_base: 17.89
Stealth Pun: Delta: 5.23. GPT4_base: 8.51 GPT3_base: 3.28
Driven to Suicide: Delta: 5.07. GPT4_base: 47.72 GPT3_base: 42.65
Foreshadowing: Delta: 5.07. GPT4_base: 42.41 GPT3_base: 37.34
Exact Words: Delta: 4.44. GPT4_base: 10.0 GPT3_base: 5.56
Big Damn Heroes: Delta: 4.17. GPT4_base: 26.75 GPT3_base: 22.58
Deadpan Snarker: Delta: 4.15. GPT4_base: 23.79 GPT3_base: 19.64
Laser-Guided Karma: Delta: 4.11. GPT4_base: 21.08 GPT3_base: 16.97
Fanservice: Delta: 4.05. GPT4_base: 19.61 GPT3_base: 15.56
Cassandra Truth: Delta: 3.84. GPT4_base: 19.49 GPT3_base: 15.65
Karmic Death: Delta: 3.47. GPT4_base: 23.68 GPT3_base: 20.21
Pet the Dog: Delta: 3.17. GPT4_base: 23.62 GPT3_base: 20.45
Black Comedy: Delta: 3.06. GPT4_base: 28.99 GPT3_base: 25.93
Jerk with a Heart of Gold: Delta: 2.69. GPT4_base: 33.74 GPT3_base: 31.05
Does This Remind You of Anything?: Delta: 2.11. GPT4_base: 11.2 GPT3_base: 9.09
Cool Car: Delta: 2.05. GPT4_base: 41.18 GPT3_base: 39.13
Police are Useless: Delta: 0.75. GPT4_base: 24.11 GPT3_base: 23.36
Comically Missing the Point: Delta: 0.48. GPT4_base: 23.21 GPT3_base: 22.73
Papa Wolf: Delta: 0.4. GPT4_base: 28.57 GPT3_base: 28.17
Crapsack World: Delta: 0.37. GPT4_base: 22.22 GPT3_base: 21.85
Disappeared Dad: Delta: 0.05. GPT4_base: 19.69 GPT3_base: 19.64
Meaningful Echo: Delta: -0.79. GPT4_base: 11.54 GPT3_base: 12.33
Body Horror: Delta: -0.83. GPT4_base: 25.74 GPT3_base: 26.57
Reasonable Authority Figure: Delta: -0.88. GPT4_base: 19.93 GPT3_base: 20.81
Adult Fear: Delta: -0.93. GPT4_base: 24.07 GPT3_base: 25.0
Hypocritical Humor: Delta: -0.97. GPT4_base: 12.82 GPT3_base: 13.79
Bittersweet Ending: Delta: -1.14. GPT4_base: 33.43 GPT3_base: 34.57
Brick Joke: Delta: -1.46. GPT4_base: 14.29 GPT3_base: 15.75
The Dragon: Delta: -1.57. GPT4_base: 26.75 GPT3_base: 28.32
Nice Job Breaking It, Hero!: Delta: -2.07. GPT4_base: 20.83 GPT3_base: 22.9
The Reveal: Delta: -2.2. GPT4_base: 17.33 GPT3_base: 19.53
Earn Your Happy Ending: Delta: -2.25. GPT4_base: 20.09 GPT3_base: 22.34
Idiot Ball: Delta: -2.76. GPT4_base: 10.32 GPT3_base: 13.08
Action Girl: Delta: -3.44. GPT4_base: 25.36 GPT3_base: 28.8
Determinator: Delta: -3.64. GPT4_base: 12.09 GPT3_base: 15.73
Took a Level in Badass: Delta: -3.86. GPT4_base: 16.0 GPT3_base: 19.86
Ironic Echo: Delta: -4.72. GPT4_base: 14.43 GPT3_base: 19.15
Chekhov's Gunman: Delta: -5.2. GPT4_base: 6.56 GPT3_base: 11.76
Chekhov's Gun: Delta: -5.32. GPT4_base: 30.38 GPT3_base: 35.7
The Alcoholic: Delta: -6.11. GPT4_base: 38.57 GPT3_base: 44.68
Anti-Hero: Delta: -6.32. GPT4_base: 15.69 GPT3_base: 22.01
Big "NO!": Delta: -7.87. GPT4_base: 9.52 GPT3_base: 17.39
Jerkass Has a Point: Delta: -10.88. GPT4_base: 6.9 GPT3_base: 17.78

==> data/Delta_GPT4base_MSRRN.tex <==
The Alcoholic: Delta: 35.58. GPT4: 38.57 MSRRN: 2.99
Cool Car: Delta: 30.98. GPT4: 41.18 MSRRN: 10.2
Downer Ending: Delta: 29.78. GPT4: 55.44 MSRRN: 25.66
Driven to Suicide: Delta: 29.07. GPT4: 47.72 MSRRN: 18.65
Abusive Parents: Delta: 28.31. GPT4: 45.45 MSRRN: 17.14
Off with His Head!: Delta: 27.93. GPT4: 46.51 MSRRN: 18.58
Roaring Rampage of Revenge: Delta: 26.58. GPT4: 37.27 MSRRN: 10.69
Red Herring: Delta: 25.66. GPT4: 31.91 MSRRN: 6.25
Disney Villain Death: Delta: 22.78. GPT4: 40.96 MSRRN: 18.18
Heel Face Turn: Delta: 19.72. GPT4: 33.33 MSRRN: 13.61
Black Comedy: Delta: 19.37. GPT4: 28.99 MSRRN: 9.62
Impaled with Extreme Prejudice: Delta: 19.12. GPT4: 42.42 MSRRN: 23.3
Smug Snake: Delta: 18.36. GPT4: 33.33 MSRRN: 14.97
Papa Wolf: Delta: 18.04. GPT4: 28.57 MSRRN: 10.53
Batman Gambit: Delta: 17.26. GPT4: 32.26 MSRRN: 15.0
Your Cheating Heart: Delta: 16.56. GPT4: 35.96 MSRRN: 19.4
Cluster F-Bomb: Delta: 16.28. GPT4: 22.22 MSRRN: 5.94
Would Hurt a Child: Delta: 16.21. GPT4: 28.57 MSRRN: 12.36
Heroic Sacrifice: Delta: 15.86. GPT4: 37.62 MSRRN: 21.76
Only Sane Man: Delta: 15.59. GPT4: 23.53 MSRRN: 7.94
Adorkable: Delta: 14.92. GPT4: 31.25 MSRRN: 16.33
Crapsack World: Delta: 14.6. GPT4: 22.22 MSRRN: 7.62
Ax-Crazy: Delta: 14.11. GPT4: 39.52 MSRRN: 25.41
Laser-Guided Karma: Delta: 13.21. GPT4: 21.08 MSRRN: 7.87
Jerk with a Heart of Gold: Delta: 13.19. GPT4: 33.74 MSRRN: 20.55
Eye Scream: Delta: 12.69. GPT4: 45.45 MSRRN: 32.76
Villainous Breakdown: Delta: 12.44. GPT4: 30.0 MSRRN: 17.56
Disproportionate Retribution: Delta: 12.16. GPT4: 26.34 MSRRN: 14.18
Would Hit a Girl: Delta: 12.14. GPT4: 15.27 MSRRN: 3.12
Earn Your Happy Ending: Delta: 11.93. GPT4: 20.09 MSRRN: 8.16
Reasonable Authority Figure: Delta: 11.33. GPT4: 19.93 MSRRN: 8.6
Affably Evil: Delta: 10.98. GPT4: 28.32 MSRRN: 17.34
Fan Disservice: Delta: 10.73. GPT4: 29.36 MSRRN: 18.63
Hope Spot: Delta: 10.47. GPT4: 33.09 MSRRN: 22.62
Karmic Death: Delta: 10.44. GPT4: 23.68 MSRRN: 13.24
Cassandra Truth: Delta: 10.23. GPT4: 19.49 MSRRN: 9.26
Karma Houdini: Delta: 10.05. GPT4: 32.16 MSRRN: 22.11
Determinator: Delta: 9.79. GPT4: 12.09 MSRRN: 2.3
Curb-Stomp Battle: Delta: 9.36. GPT4: 31.58 MSRRN: 22.22
Chekhov's Skill: Delta: 9.29. GPT4: 25.88 MSRRN: 16.59
Disappeared Dad: Delta: 8.06. GPT4: 19.69 MSRRN: 11.63
Faux Affably Evil: Delta: 7.62. GPT4: 27.03 MSRRN: 19.41
Heroic BSoD: Delta: 7.51. GPT4: 27.87 MSRRN: 20.36
 "The Reason You Suck" Speech: Delta: 7.43. GPT4: 31.9 MSRRN: 24.47
Freudian Excuse: Delta: 7.27. GPT4: 15.69 MSRRN: 8.42
Asshole Victim: Delta: 7.2. GPT4: 37.61 MSRRN: 30.41
Butt-Monkey: Delta: 6.99. GPT4: 28.25 MSRRN: 21.26
Comically Missing the Point: Delta: 6.02. GPT4: 23.21 MSRRN: 17.19
Ms. Fanservice: Delta: 6.01. GPT4: 23.44 MSRRN: 17.43
Pet the Dog: Delta: 5.59. GPT4: 23.62 MSRRN: 18.03
Police are Useless: Delta: 5.49. GPT4: 24.11 MSRRN: 18.62
Action Girl: Delta: 5.48. GPT4: 25.36 MSRRN: 19.88
Kick the Dog: Delta: 5.47. GPT4: 30.47 MSRRN: 25.0
Took a Level in Badass: Delta: 5.31. GPT4: 16.0 MSRRN: 10.69
Badass Boast: Delta: 5.31. GPT4: 25.0 MSRRN: 19.69
Bittersweet Ending: Delta: 4.73. GPT4: 33.43 MSRRN: 28.7
Blatant Lies: Delta: 4.43. GPT4: 16.19 MSRRN: 11.76
Too Dumb to Live: Delta: 3.44. GPT4: 31.47 MSRRN: 28.03
Foreshadowing: Delta: 3.37. GPT4: 42.41 MSRRN: 39.04
Anti-Hero: Delta: 3.06. GPT4: 15.69 MSRRN: 12.63
Jerkass: Delta: 2.88. GPT4: 33.82 MSRRN: 30.94
The Dragon: Delta: 2.87. GPT4: 26.75 MSRRN: 23.88
Gory Discretion Shot: Delta: 2.83. GPT4: 24.53 MSRRN: 21.7
Big Damn Heroes: Delta: 2.8. GPT4: 26.75 MSRRN: 23.95
Oh, Crap!: Delta: 2.68. GPT4: 41.35 MSRRN: 38.67
Body Horror: Delta: 2.55. GPT4: 25.74 MSRRN: 23.19
Screw This, I'm Outta Here!: Delta: 2.44. GPT4: 21.01 MSRRN: 18.57
Berserk Button: Delta: 2.42. GPT4: 28.46 MSRRN: 26.04
My God, What Have I Done?: Delta: 2.2. GPT4: 24.07 MSRRN: 21.88
What the Hell, Hero?: Delta: 2.12. GPT4: 19.23 MSRRN: 17.11
The Reveal: Delta: 1.37. GPT4: 17.33 MSRRN: 15.96
Irony: Delta: 1.2. GPT4: 17.03 MSRRN: 15.83
Fanservice: Delta: 1.11. GPT4: 19.61 MSRRN: 18.5
Adult Fear: Delta: 0.92. GPT4: 24.07 MSRRN: 23.15
Hoist by His Own Petard: Delta: 0.37. GPT4: 28.8 MSRRN: 28.43
Not So Different: Delta: 0.13. GPT4: 23.17 MSRRN: 23.04
Big Bad: Delta: -0.16. GPT4: 38.0 MSRRN: 38.16
Meaningful Echo: Delta: -2.14. GPT4: 11.54 MSRRN: 13.68
Exact Words: Delta: -2.39. GPT4: 10.0 MSRRN: 12.39
Even Evil Has Standards: Delta: -5.15. GPT4: 23.21 MSRRN: 28.36
Nice Job Breaking It, Hero!: Delta: -5.26. GPT4: 20.83 MSRRN: 26.09
Stealth Pun: Delta: -6.3. GPT4: 8.51 MSRRN: 14.81
Groin Attack: Delta: -6.61. GPT4: 16.0 MSRRN: 22.61
Does This Remind You of Anything?: Delta: -6.71. GPT4: 11.2 MSRRN: 17.91
Tempting Fate: Delta: -7.33. GPT4: 18.07 MSRRN: 25.4
Ironic Echo: Delta: -7.97. GPT4: 14.43 MSRRN: 22.4
Jerkass Has a Point: Delta: -9.46. GPT4: 6.9 MSRRN: 16.36
Chekhov's Gun: Delta: -9.62. GPT4: 30.38 MSRRN: 40.0
Chekhov's Gunman: Delta: -9.86. GPT4: 6.56 MSRRN: 16.42
Precision F-Strike: Delta: -10.4. GPT4: 8.33 MSRRN: 18.73
Deadpan Snarker: Delta: -10.7. GPT4: 23.79 MSRRN: 34.49
Hypocritical Humor: Delta: -11.04. GPT4: 12.82 MSRRN: 23.86
Idiot Ball: Delta: -12.36. GPT4: 10.32 MSRRN: 22.68
Big "NO!": Delta: -12.7. GPT4: 9.52 MSRRN: 22.22
Brick Joke: Delta: -14.75. GPT4: 14.29 MSRRN: 29.04

==> data/GPT4_base_PerTropeF1.tex <==
("Chekhov's Gunman", 6.56)
('Jerkass Has a Point', 6.9)
('Precision F-Strike', 8.33)
('Stealth Pun', 8.51)
('Big \\"NO!\\"', 9.52)
('Exact Words', 10.0)
('Idiot Ball', 10.32)
('Does This Remind You of Anything?', 11.2)
('Meaningful Echo', 11.54)
('Determinator', 12.09)
('Hypocritical Humor', 12.82)
('Brick Joke', 14.29)
('Ironic Echo', 14.43)
('Would Hit a Girl', 15.27)
('Anti-Hero', 15.69)
('Freudian Excuse', 15.69)
('Groin Attack', 16.0)
('Took a Level in Badass', 16.0)
('Blatant Lies', 16.19)
('Irony', 17.03)
('The Reveal', 17.33)
('Tempting Fate', 18.07)
('What the Hell, Hero?', 19.23)
('Cassandra Truth', 19.49)
('Fanservice', 19.61)
('Disappeared Dad', 19.69)
('Reasonable Authority Figure', 19.93)
('Earn Your Happy Ending', 20.09)
('Nice Job Breaking It, Hero!', 20.83)
("Screw This, I'm Outta Here!", 21.01)
('Laser-Guided Karma', 21.08)
('Cluster F-Bomb', 22.22)
('Crapsack World', 22.22)
('Not So Different', 23.17)
('Even Evil Has Standards', 23.21)
('Comically Missing the Point', 23.21)
('Ms. Fanservice', 23.44)
('Only Sane Man', 23.53)
('Pet the Dog', 23.62)
('Karmic Death', 23.68)
('Deadpan Snarker', 23.79)
('Adult Fear', 24.07)
('My God, What Have I Done?', 24.07)
('Police are Useless', 24.11)
('Gory Discretion Shot', 24.53)
('Badass Boast', 25.0)
('Action Girl', 25.36)
('Body Horror', 25.74)
("Chekhov's Skill", 25.88)
('Disproportionate Retribution', 26.34)
('Big Damn Heroes', 26.75)
('The Dragon', 26.75)
('Faux Affably Evil', 27.03)
('Heroic BSoD', 27.87)
('Butt-Monkey', 28.25)
('Affably Evil', 28.32)
('Berserk Button', 28.46)
('Would Hurt a Child', 28.57)
('Papa Wolf', 28.57)
('Hoist by His Own Petard', 28.8)
('Black Comedy', 28.99)
('Fan Disservice', 29.36)
('Villainous Breakdown', 30.0)
("Chekhov's Gun", 30.38)
('Kick the Dog', 30.47)
('Adorkable', 31.25)
('Too Dumb to Live', 31.47)
('Curb-Stomp Battle', 31.58)
('\\"The Reason You Suck\\" Speech', 31.9)
('Red Herring', 31.91)
('Karma Houdini', 32.16)
('Batman Gambit', 32.26)
('Hope Spot', 33.09)
('Smug Snake', 33.33)
('Heel Face Turn', 33.33)
('Bittersweet Ending', 33.43)
('Jerk with a Heart of Gold', 33.74)
('Jerkass', 33.82)
('Your Cheating Heart', 35.96)
('Roaring Rampage of Revenge', 37.27)
('Asshole Victim', 37.61)
('Heroic Sacrifice', 37.62)
('Big Bad', 38.0)
('The Alcoholic', 38.57)
('Ax-Crazy', 39.52)
('Disney Villain Death', 40.96)
('Cool Car', 41.18)
('Oh, Crap!', 41.35)
('Foreshadowing', 42.41)
('Impaled with Extreme Prejudice', 42.42)
('Abusive Parents', 45.45)
('Eye Scream', 45.45)
('Off with His Head!', 46.51)
('Driven to Suicide', 47.72)
('Downer Ending', 55.44)


==> data/GPT4_base_PerTropePrecision.tex <==
('Determinator', 6.47)
('Anti-Hero', 8.7)
('Would Hit a Girl', 8.7)
('Idiot Ball', 8.7)
('Took a Level in Badass', 9.01)
('The Reveal', 9.61)
('Blatant Lies', 10.15)
('Irony', 10.31)
('Does This Remind You of Anything?', 10.45)
('Jerkass Has a Point', 11.11)
('Freudian Excuse', 11.32)
('Earn Your Happy Ending', 11.42)
("Chekhov's Gunman", 11.76)
('Reasonable Authority Figure', 12.17)
('Laser-Guided Karma', 12.22)
('Cassandra Truth', 12.5)
('Disappeared Dad', 12.67)
('Tempting Fate', 13.39)
('Crapsack World', 13.53)
('Karmic Death', 14.01)
('Adult Fear', 14.07)
("Screw This, I'm Outta Here!", 14.2)
('Nice Job Breaking It, Hero!', 14.53)
('Exact Words', 15.0)
('Action Girl', 15.22)
('Precision F-Strike', 16.0)
('Police are Useless', 16.36)
('Body Horror', 16.46)
('Big Damn Heroes', 16.54)
('Pet the Dog', 17.44)
('My God, What Have I Done?', 17.69)
('Disproportionate Retribution', 17.98)
('Not So Different', 18.81)
('Would Hurt a Child', 19.12)
('Heroic BSoD', 19.21)
('Faux Affably Evil', 19.23)
('Villainous Breakdown', 19.25)
('Comically Missing the Point', 19.4)
('Hoist by His Own Petard', 19.57)
('Papa Wolf', 19.61)
('The Dragon', 19.63)
('Only Sane Man', 20.0)
('Fanservice', 20.0)
('What the Hell, Hero?', 20.0)
('Kick the Dog', 20.52)
('Bittersweet Ending', 21.22)
('Batman Gambit', 21.74)
('Smug Snake', 22.5)
('Jerkass', 22.69)
('Black Comedy', 23.26)
('Ms. Fanservice', 23.44)
('Butt-Monkey', 23.58)
('Berserk Button', 24.31)
('Big Bad', 24.63)
('Meaningful Echo', 25.0)
('Your Cheating Heart', 25.15)
('Adorkable', 25.32)
('Asshole Victim', 26.51)
('Roaring Rampage of Revenge', 26.55)
('Oh, Crap!', 27.13)
('Heel Face Turn', 27.37)
('Jerk with a Heart of Gold', 27.52)
('Affably Evil', 27.59)
('Gory Discretion Shot', 27.66)
('\\"The Reason You Suck\\" Speech', 27.66)
('Hypocritical Humor', 27.78)
('Heroic Sacrifice', 28.36)
('Ax-Crazy', 28.99)
('The Alcoholic', 29.03)
('Hope Spot', 29.49)
('Curb-Stomp Battle', 30.0)
('Too Dumb to Live', 30.39)
('Red Herring', 30.61)
('Fan Disservice', 31.37)
('Karma Houdini', 32.32)
('Disney Villain Death', 32.69)
('Even Evil Has Standards', 33.33)
('Cool Car', 33.87)
('Deadpan Snarker', 36.0)
('Abusive Parents', 37.04)
("Chekhov's Gun", 37.21)
('Driven to Suicide', 37.3)
('Impaled with Extreme Prejudice', 37.5)
('Foreshadowing', 37.61)
("Chekhov's Skill", 39.29)
('Downer Ending', 41.36)
('Off with His Head!', 41.67)
('Big \\"NO!\\"', 42.86)
('Groin Attack', 44.44)
('Badass Boast', 45.45)
('Brick Joke', 50.0)
('Stealth Pun', 50.0)
('Cluster F-Bomb', 55.56)
('Eye Scream', 62.5)
('Ironic Echo', 63.64)


==> data/GPT4_base_preTropeRecall.tex <==
("Chekhov's Gunman", 4.55)
('Stealth Pun', 4.65)
('Jerkass Has a Point', 5.0)
('Big \\"NO!\\"', 5.36)
('Precision F-Strike', 5.63)
('Exact Words', 7.5)
('Meaningful Echo', 7.5)
('Ironic Echo', 8.14)
('Brick Joke', 8.33)
('Hypocritical Humor', 8.33)
('Groin Attack', 9.76)
('Does This Remind You of Anything?', 12.07)
('Idiot Ball', 12.7)
('Cluster F-Bomb', 13.89)
('Badass Boast', 17.24)
('Deadpan Snarker', 17.76)
('Even Evil Has Standards', 17.81)
('What the Hell, Hero?', 18.52)
('Fanservice', 19.23)
("Chekhov's Skill", 19.3)
('Gory Discretion Shot', 22.03)
('Ms. Fanservice', 23.44)
('Freudian Excuse', 25.53)
("Chekhov's Gun", 25.67)
('Fan Disservice', 27.59)
('Tempting Fate', 27.78)
('Only Sane Man', 28.57)
('Comically Missing the Point', 28.89)
('Affably Evil', 29.09)
('Not So Different', 30.16)
('Karma Houdini', 32.0)
('Too Dumb to Live', 32.63)
('Curb-Stomp Battle', 33.33)
('Red Herring', 33.33)
('Berserk Button', 34.31)
('Butt-Monkey', 35.21)
('Eye Scream', 35.71)
('Pet the Dog', 36.59)
('Nice Job Breaking It, Hero!', 36.76)
('\\"The Reason You Suck\\" Speech', 37.68)
('My God, What Have I Done?', 37.68)
('Hope Spot', 37.7)
('Black Comedy', 38.46)
('Blatant Lies', 40.0)
("Screw This, I'm Outta Here!", 40.32)
('Adorkable', 40.82)
('The Dragon', 42.0)
('Heel Face Turn', 42.62)
('Jerk with a Heart of Gold', 43.62)
('Disappeared Dad', 44.19)
('Cassandra Truth', 44.19)
('Faux Affably Evil', 45.45)
('Police are Useless', 45.76)
('Foreshadowing', 48.62)
('Impaled with Extreme Prejudice', 48.84)
('Irony', 49.09)
('Disproportionate Retribution', 49.23)
('Heroic BSoD', 50.75)
('Cool Car', 52.5)
('Papa Wolf', 52.63)
('Off with His Head!', 52.63)
('Hoist by His Own Petard', 54.55)
('Disney Villain Death', 54.84)
('Reasonable Authority Figure', 54.9)
('Heroic Sacrifice', 55.88)
('Would Hurt a Child', 56.52)
('The Alcoholic', 57.45)
('Abusive Parents', 58.82)
('Body Horror', 59.09)
('Kick the Dog', 59.14)
('Ax-Crazy', 62.03)
('Crapsack World', 62.22)
('Would Hit a Girl', 62.5)
('Roaring Rampage of Revenge', 62.5)
('Batman Gambit', 62.5)
('Your Cheating Heart', 63.08)
('Smug Snake', 64.29)
('Asshole Victim', 64.71)
('Driven to Suicide', 66.2)
('Jerkass', 66.39)
('Villainous Breakdown', 67.92)
('Big Damn Heroes', 69.84)
('Took a Level in Badass', 71.43)
('Action Girl', 76.09)
('Karmic Death', 76.6)
('Laser-Guided Karma', 76.79)
('Bittersweet Ending', 78.72)
('Anti-Hero', 80.0)
('Big Bad', 83.1)
('Adult Fear', 83.33)
('Earn Your Happy Ending', 83.33)
('Downer Ending', 84.04)
('Oh, Crap!', 86.93)
('The Reveal', 87.69)
('Determinator', 91.67)

==> data/MSRRN_PerTrope.tex <==
("Chekhov's Gun", 0.4),
 ('Foreshadowing', 0.3904034896401309),
 ('Oh, Crap!', 0.3867069486404834),
 ('Big Bad', 0.3815789473684211),
 ('Deadpan Snarker', 0.3449275362318841),
 ('Eye Scream', 0.32764505119453924),
 ('Jerkass', 0.3093525179856115),
 ('Asshole Victim', 0.30406852248394),
 ('Brick Joke', 0.29041095890410956),
 ('Bittersweet Ending', 0.28699551569506726),
 ('Hoist by His Own Petard', 0.28431372549019607),
 ('Even Evil Has Standards', 0.2835820895522388),
 ('Too Dumb to Live', 0.28028503562945367),
 ('Nice Job Breaking It, Hero!', 0.26086956521739135),
 ('Berserk Button', 0.26035502958579887),
 ('Downer Ending', 0.256578947368421),
 ('Ax-Crazy', 0.254054054054054),
 ('Tempting Fate', 0.25396825396825395),
 ('Kick the Dog', 0.24999999999999994),
 (' "The Reason You Suck" Speech', 0.24472573839662445),
 ('Big Damn Heroes', 0.23948220064724918),
 ('The Dragon', 0.23880597014925373),
 ('Hypocritical Humor', 0.23863636363636362),
 ('all', 0.23576985627005406),
 ('Impaled with Extreme Prejudice', 0.23300970873786409),
 ('Body Horror', 0.2318840579710145),
 ('Adult Fear', 0.23151125401929262),
 ('Not So Different', 0.23036649214659688),
 ('Idiot Ball', 0.22680412371134023),
 ('Hope Spot', 0.22619047619047616),
 ('Groin Attack', 0.22613065326633167),
 ('Ironic Echo', 0.224),
 ('Curb-Stomp Battle', 0.22222222222222224),
 ('Big "NO!"', 0.22222222222222224),
 ('Karma Houdini', 0.22113022113022107),
 ('My God, What Have I Done?', 0.21875),
 ('Heroic Sacrifice', 0.2175732217573222),
 ('Gory Discretion Shot', 0.2169811320754717),
 ('Butt-Monkey', 0.21256038647342992),
 ('Jerk with a Heart of Gold', 0.20547945205479454),
 ('Heroic BSoD', 0.2035928143712575),
 ('Action Girl', 0.1987577639751553),
 ('Badass Boast', 0.19689119170984454),
 ('Faux Affably Evil', 0.1940928270042194),
 ('Your Cheating Heart', 0.19399538106235564),
 ('Precision F-Strike', 0.18732782369146003),
 ('Driven to Suicide', 0.1864801864801865),
 ('Fan Disservice', 0.18627450980392157),
 ('Police are Useless', 0.18620689655172412),
 ('Off with His Head!', 0.18579234972677594),
 ("Screw This, I'm Outta Here!", 0.18571428571428572),
 ('Fanservice', 0.185),
 ('Disney Villain Death', 0.18181818181818182),
 ('Pet the Dog', 0.18032786885245905),
 ('Does This Remind You of Anything?', 0.1791044776119403),
 ('Villainous Breakdown', 0.175609756097561),
 ('Ms. Fanservice', 0.1743119266055046),
 ('Affably Evil', 0.17341040462427745),
 ('Comically Missing the Point', 0.17187500000000003),
 ('Abusive Parents', 0.17142857142857143),
 ('What the Hell, Hero?', 0.1711229946524064),
 ("Chekhov's Skill", 0.16585365853658537),
 ("Chekhov's Gunman", 0.16417910447761194),
 ('Jerkass Has a Point', 0.16363636363636366),
 ('Adorkable', 0.16326530612244897),
 ('The Reveal', 0.1595744680851064),
 ('Irony', 0.15827338129496404),
 ('Batman Gambit', 0.15),
 ('Smug Snake', 0.14965986394557823),
 ('Stealth Pun', 0.14814814814814814),
 ('Disproportionate Retribution', 0.14184397163120566),
 ('Meaningful Echo', 0.13675213675213674),
 ('Heel Face Turn', 0.13612565445026178),
 ('Karmic Death', 0.1323529411764706),
 ('Anti-Hero', 0.1263157894736842),
 ('Exact Words', 0.1238938053097345),
 ('Would Hurt a Child', 0.12359550561797751),
 ('Blatant Lies', 0.11764705882352941),
 ('Disappeared Dad', 0.11627906976744186),
 ('Took a Level in Badass', 0.1068702290076336),
 ('Roaring Rampage of Revenge', 0.10687022900763359),
 ('Papa Wolf', 0.10526315789473684),
 ('Cool Car', 0.1020408163265306),
 ('Black Comedy', 0.09615384615384615),
 ('Cassandra Truth', 0.09259259259259257),
 ('Reasonable Authority Figure', 0.08602150537634409),
 ('Freudian Excuse', 0.08421052631578947),
 ('Earn Your Happy Ending', 0.08163265306122448),
 ('Only Sane Man', 0.07936507936507935),
 ('Laser-Guided Karma', 0.07874015748031496),
 ('Crapsack World', 0.0761904761904762),
 ('Red Herring', 0.0625),
 ('Cluster F-Bomb', 0.0594059405940594),
 ('Would Hit a Girl', 0.03125),
 ('The Alcoholic', 0.029850746268656716),
 ('Determinator', 0.022988505747126433)

==> data/attack.tex <==
Sentence:
 "Big Bad":["After Charlie and Itchy fail several times to get the stolen goods from Carface, it is revealed that he is working for Annabelle's evil cousin, Belladonna, who plots to use a massive version of the hypnotic dog whistle to hypnotize every dog in San Francisco into stealing the masters' Christmas presents, causing them to be thrown out of their houses and abandoned."],
 "Blatant Lies":['Not wanting Mitch to realize the lengths to which she went to get his attention, she lies and tells him that her primary reason for coming to Bodega Bay was to visit Annie, a friend of hers from school.'],
 "Bittersweet Ending":['The film ends with Pauline being arrested after protesting and refusing to continue but before she can be put on trial, she is captured by the resurgent British Resistance and agrees to work for them as they fight to liberate the country with the help of arriving American troops.']}

CoT_plot = {
    "Big Bad":['MoonOverMiami', 'StarterFor10', 'Secretariat', 'CantHardlyWait', 'MarleyAndMe', 'Evita', 'WeWereSoldiers', 'TheChristmasToy', 'ShatteredGlass', 'StuckInLove', 'NightMoves', 'TheDevilsArithmetic', 'QuickChange', 'Ararat', 'WhistleDownTheWind', 'FindingNeverland', 'BlackSnakeMoan', 'Poseidon', 'SnowCake', 'BlackSea', 'HeadOfState', 'Twister', 'ItHappenedHere', 'TheIncredibleShrinkingMan', 'TheAmericanPresident', 'W', 'Goodfellas', 'RabbitFire', 'CoolRunnings', 'HeartsInAtlantis'],   
    "Blatant Lies":['JesusChristVampireHunter', 'AnAllDogsChristmasCarol', 'HigherLearning', 'CloakAndDagger', 'WhistleDownTheWind', 'TheAngelsShare', 'BartonFink', 'DeadAndDeader', 'NightMoves', 'QuickChange', 'BlackSnakeMoan', 'FromBeyond', 'Sleepwalkers', 'TheAdventuresOfPlutoNash', 'CloudAtlas', 'StreetsOfFire', 'FindingNeverland', 'CatsEye', 'TheTenCommandments', 'TheEagleHasLanded', 'CoolRunnings', 'Evita', 'WeWereSoldiers', 'MissionImpossibleII', 'Poseidon', 'Goodfellas', 'NancyDrew', 'InvasionOfTheBodySnatchers', 'SnowCake', 'TheIncredibleShrinkingMan'],
    "Kick the Dog":['CloakAndDagger', 'MarleyAndMe', 'FuneralInBerlin', 'RabbitFire', 'LakePlacid3', 'Horsemen', 'Ararat', 'CoolRunnings', 'Poseidon', 'Evita', 'NightMoves', 'ScaryMovie', 'ShatteredGlass', 'HeadOfState', 'WeWereSoldiers', 'SnowCake', 'LittleRuralRidingHood', 'WhistleDownTheWind', 'TheAmericanPresident', 'TheIncredibleShrinkingMan', 'W', 'TheChristmasToy', 'DeadSpaceDownfall', 'FromBeyond', 'BartonFink', 'QuickChange', 'FindingNeverland', 'Twister', 'InvasionOfTheBodySnatchers', 'NancyDrew']
}




==> data/backup.tex <==
    \begin{itemize}
    \item Survey:Reasoning with Language Model Prompting: A Survey %https://arxiv.org/pdf/2212.09597.pdf
    \item Towards Reasoning in Large Language Models: A Survey % https://arxiv.org/pdf/2212.10403.pdf
    \end{itemize}

    \begin{itemize}
    \item Commonsense Reasoning
    
CommonsenseQA 2.0: Exposing the Limits of AI through Gamification \cite{CommonsenseQA}

CROW: Benchmarking Commonsense Reasoning in Real-World Tasks \cite{ismayilzada2023crow}

    \item Mathematical Reasoning
    
PAL: Program-aided Language Models\cite{gao2022pal}

    \item Logical Reasoning
    
Language Models Are Greedy Reasoners: A Systematic Formal Analysis of Chain-of-Thought\cite{PrOntoQA}

\end{itemize}

==> data/subset.tex <==
% trope = ['Kick the Dog','Big Bad','What the Hell, Hero?', "Chekhov's Gunman", 'Irony', 'Determinator', "Screw This, I'm Outta Here!",'Adorkable', 'Adult Fear', 'Too Dumb to Live', 'Deadpan Snarker', 'Would Hurt a Child','Eye Scream','Stealth Pun', 'Not So Different','Bittersweet Ending','Only Sane Man','Smug Snake','Red Herring','Blatant Lies']

% plot =  ['ClubDread', 'Taken', 'ScarletStreet', 'Hook', 'Poseidon', 'DeadAndDeader', 'TheShawshankRedemption', 'AGoodYear', 'CatsEye', 'EnemyMine', 'ExitWounds', 'Ararat', 'BlackSnakeMoan', 'Dragonslayer', 'RabbitFire', 'Stagecoach', 'QuickChange', 'CantHardlyWait', 'TheEagleHasLanded', 'TheTenCommandments', 'FromBeyond', 'StarTrekGenerations', 'NightAndTheCity', 'BachelorMother', 'ItHappenedHere', 'HatchetII', 'WeWereSoldiers', 'Doomsday', 'FuneralInBerlin', 'Willow', 'TopDog', 'TheAmericanPresident', 'MurderParty', 'Topper', 'WhistleDownTheWind', 'CoolRunnings', 'HeadOfState', 'TheAngelsShare', 'CloakAndDagger', 'ZabriskiePoint', 'SnowCake', 'TheChangeling', 'LittleRuralRidingHood', 'KillBillVol2', 'TheIncredibleShrinkingMan', 'LastManStanding', 'AvatarTheLastAirbender', 'KnockKnock', 'TheAdventuresOfPlutoNash', 'JesusChristVampireHunter', 'TheDevilsArithmetic', 'HeartsInAtlantis', 'WildTarget', 'NancyDrew', 'Outbreak', 'Twister', 'ShadowOfADoubt', 'StuckInLove', 'Sleepwalkers', 'PrettyBaby', 'Evita', 'WildAtHeart', 'Crazy', 'Tarantula', 'TheBirds', 'InvasionOfTheBodySnatchers', 'DeadSpaceDownfall', 'CloudAtlas', 'SevenChances', 'MoonOverMiami', 'TheMuppets', 'SpiritStallionOfTheCimarron', 'BartonFink', 'W', 'StarterFor10', 'TheChristmasToy', 'FatalAttraction', 'MarleyAndMe', 'Sorcerer', 'BrewstersMillions', 'ChildsPlay2', 'KangarooJack', 'BlackSea', 'DropDeadGorgeous', 'EuropaEuropa', 'SmallTimeCrooks', 'Horsemen', 'StreetsOfFire', 'NightMoves', 'AnAllDogsChristmasCarol', 'TheShallows', 'BillyMadison', 'TheLostWorldJurassicPark', 'Anaconda', 'HospitalMassacre', 'MissionImpossibleII', 'DanInRealLife', 'LakePlacid3', 'TheTroubleWithHarry', 'TheBraveLittleToaster']

% plot = ['TheShallows', 'W', 'Stagecoach', 'StarTrekGenerations', 'JesusChristVampireHunter', 'NightAndTheCity', 'WildTarget', 'TopDog', 'TheEagleHasLanded', 'TheChangeling', 'HospitalMassacre', 'Poseidon', 'Sleepwalkers', 'FromBeyond', 'Secretariat', 'EnemyMine', 'TheBraveLittleToaster', 'ExitWounds', 'SpiritStallionOfTheCimarron', 'CantHardlyWait', 'MoonOverMiami', 'DropDeadGorgeous', 'BachelorMother', 'TheTenCommandments', 'SevenChances', 'BillyMadison', 'ItHappenedHere', 'HigherLearning', 'FuneralInBerlin', 'Crazy', 'MarleyAndMe', 'HatchetII', 'WeWereSoldiers', 'QuickChange', 'Taken', 'ShadowOfADoubt', 'AvatarTheLastAirbender', 'Sorcerer', 'TheGingerdeadMan', 'Horsemen', 'HeadOfState', 'BlackSnakeMoan', 'WhistleDownTheWind', 'InvasionOfTheBodySnatchers', 'SmallTimeCrooks', 'TheMuppets', 'DanInRealLife', 'PrettyBaby', 'Goodfellas', 'NightMoves', 'FindingNeverland', 'DeadSpaceDownfall', 'Tarantula', 'TheIncredibleShrinkingMan', 'KillBillVol2', 'TheAdventuresOfPlutoNash', 'SnowCake', 'BartonFink', 'CloudAtlas', 'Twister', 'NancyDrew', 'TheShawshankRedemption', 'TheBirds', 'Anaconda', 'KnockKnock', 'Ararat', 'Topper', 'AGoodYear', 'RabbitFire', 'TheAngelsShare', 'SomethingBorrowed', 'TheTroubleWithHarry', 'AnAllDogsChristmasCarol', 'FatalAttraction', 'AlienCovenant', 'HeartsInAtlantis', 'EuropaEuropa', 'OceansEleven', 'ZabriskiePoint', 'KangarooJack', 'WhenAKillerCalls', 'Friday', 'TheLostWorldJurassicPark', 'LittleRuralRidingHood', 'LakePlacid3', 'StuckInLove', 'War', 'LastManStanding', 'ScarletStreet', 'DeadAndDeader', 'Willow', 'WildAtHeart', 'BlackSea', 'TheChristmasToy', 'CatsEye', 'Outbreak', 'StarterFor10', 'Dragonslayer', 'StreetsOfFire', 'BrewstersMillions']

==> figures/all_distribution.tex <==
% \begin{figure}[h!]
%     \centering\includegraphics[width=\textwidth]{latex/figures/image/all_distribution.png}
%     \caption{Distribution of each trope in predicting a positive outcome differs among the three binary classification results across the entire dataset}
%     \label{fig:whole_distribution}
% \end{figure}

\begin{figure}[ht]
  \begin{adjustbox}{addcode={
  \begin{minipage}{\width}
  }{\caption{Distribution of each trope in predicting a positive outcome differs among the three binary classification results across the entire dataset}
  \end{minipage}},rotate=90,center}
      \includegraphics[scale=.3]{latex/figures/image/all_distribution.png}%
  \end{adjustbox}
\end{figure}


==> sections/z_old_backup.tex <==
In light of this, we first investigate LLMs' reasoning capability by revisiting an existing Trope in Movie Synopses (TiMoS) dataset \cite{chang2021situationtimos}. As Figure \ref{fig:figure1} shows, advanced LLMs such as GPT-4, ChatGPT, and fine-tuned LLaMa-2 perform poorly, only achieving F1 scores at the level of random guessing even when they are equipped with CoT \cite{wei2022chaincot} prompts. This suggests that state-of-the-art LLMs, despite dominating various benchmarks, do not carry reasoning skills for challenges in trope understanding tasks. In addition, evidence of LLMs lacking trope reasoning capability is apparent through several observations: (1) LLMs exhibit significantly diminished performance when tasked with navigating multiple tropes instead of a singular one (Section \ref{subsec:4:3:binaryresults}), (2) LLMs struggle notably when a trope necessitates comprehension across various plot elements (Sections \ref{subsec:4:6:difficulty}, \ref{subsec:4:8:gptvssl}, \ref{subsec:4:7:pertrope}).

In addition to assessing trope reasoning capabilities, we propose innovative approaches to evaluate LLMs and CoT's tendency for hallucination. Our findings reveal that not only do LLMs suffer from hallucination, but CoT exacerbates this tendency, resulting in worse performance compared to prompting without it. Specifically, inspired by prior reading comprehension studies \cite{jia2017adversarialsquad}, we devise an Adversarial Injection that inserts trope-related text tokens without explicit trope introduction into a movie synopsis, aimed at gauging whether LLMs are misled.
%(2) Drawing inspiration from previous VLM research \cite{mao2023doubly}, we introduce a Doubly Right Analysis, evaluating CoT's reasoning coherence to determine correctness. 
The propensity for hallucination tendency is underscored by: 
(1) a stark decline in LLM precision when employing CoT (Section \ref{subsec:4:4:cot}), 
(2) Adversarial Injection significantly misleads LLMs through keyword and pattern recognition, especially when CoT is equipped (Section \ref{subsec:4:10:attack}), and 
%(3) Doubly Right Analysis highlights instances where 
CoT generates accurate responses with erroneous rationales (Section \ref{subsec:4:9:doublyright}).

%When equipped with prompt engineering techniques such as in-context learning \cite{gpt3} and chain-of-thoughts \cite{wei2022chaincot}, LLMs can easily perform not only system 1 tasks that require only shallow semantics, but several complex reasoning tasks that seem to go beyond shallow semantics. For example, arithmetic \cite{cobbe2021traininggsm8k} that requires stepwise and compositional reasoning, commonsense \cite{talmor2019commonsenseqa} acquire not only the fact presented in the context but also commonsense knowledge, logic reasoning that needs evidence integration and commonsense knowledge. Above challenges \textit{seems} enter the field of system 2 reasoning by requiring some components of \textit{slow} reasoning such as step-by-step understanding and fusing the evidence and commonsense. These findings suggested that LLMs \textit{seems} gradually conquering traditionally considered challenging or even impossible tasks, and also raising the research question of this paper: Can LLMs perform system 2 reasoning as humans?

%These challenges appear to delve into the realm of System 2 reasoning~\cite{evans2003two}, as they require components of slower, step-by-step understanding and the integration of evidence and commonsense knowledge. These findings suggest that LLMs are gradually making strides in tackling traditionally considered challenging and even seemingly impossible tasks. This, in turn, prompts the central research question of this paper: \textit{Can LLMs perform System 2 reasoning tasks in a manner akin to humans?}
}

%When equipped with prompt engineering techniques such as in-context learning \cite{gpt3} and chain-of-thoughts \cite{wei2022chaincot}, LLMs can perform complex reasoning tasks including but not limited to arithmetic \cite{cobbe2021traininggsm8k}, commonsense \cite{talmor2019commonsenseqa} or logic \cite{liu2023logiqa} reasoning with few step-by-step examples. These findings suggested that LLMs \textit{seems} gradually conquering traditionally considered challenging or even impossible tasks, and also raising the research question of this paper: Can LLMs perform system 2 reasoning as humans?


%\xudong{it will be more friendly for audience to first introduce what is system 1 task and what is system 2 task in both abstract and introduction, considering that some audience is not familiar with the 2 system thinking theory. more importantly, is there any reference that we can refer to to convince the audience that the aforementioned tasks are only system 1?}

%narritive vs factual
%%contamination?


%Different from mostly-tackled System 1 tasks, System 2 reasoning, which requires skills of consciousness, systematic generalization, causality, and comprehension, remains challenging for advanced deep learning systems \cite{bengio2019system2}. While LLMs appear to carry significantly better reasoning skills compared to previous supervised, task-specific learning models,  it is still unclear if LLMs are able to perform System 2 reasoning.
%some examples?

%One of the core challenges in development and evaluation is the time-consuming and prohibitive nature of benchmark construction. This work is the first work that leverages \textit{tropes in movie synopses} as the testbed of System 2 reasoning skills. Tropes are storytelling devices that are frequently used in creative productions such as novels or movie stories. 

%Creating a story based on predefined tropes may appear straightforward, but identifying tropes within an existing story demands a deeper analysis. It entails unraveling the intricacies of characters' motivations, intentions, and the underlying causality of plots concealed beneath the surface of shallow semantics, symbols, and implications.
%\xudong{It is straightforward to develop a story from a given trope. However, to determine the trope given a story, one needs to thoroughly and deeply capture the core plot elements out of noisy surface-level signals and carefully reason. Generally, here I think we should hghlight why trope understanding is system-2 and why it is challenging. Context-length is another aspect we can highlight} 
%Creating a story based on predefined tropes may appear straightforward, but identifying tropes within an existing story demands a deeper analysis. It entails unraveling the intricacies of characters' motivations, intentions, and the underlying causality of plots concealed beneath the surface of shallow semantics, symbols, and implications. %Previous work \cite{chang2021situationtimos,su2021truman} confirmed that system 2 reasoning skills could be examined with tropes in movie stories and revealed a huge gap between supervised models and humans. 
%Earlier studies \cite{chang2021situationtimos,su2021truman} have validated the use of tropes in movie narratives as a means to assess System 2 reasoning skills. These studies have also underscored a substantial disparity between the performance of supervised models and human capabilities in this context.
%utilized tropes in movie stories or clips to examine System 2 reasoning skills of supervised learning systems and observed significant performance gaps between modern learning models and humans. 
%Therefore, this work revisits tropes in movies and evaluates System 2 reasoning skills of advanced LLMs.

%System 2 Reasoning Incapability is evident by (1) LLMs perform significantly worse when they need to focus on various tropes instead of a single trope (Section \ref{subsec:4:3:binaryresults}), (2) LLMs perform much worse when a trope requires understanding across more plot elements (Section \ref{subsec:4:6:difficulty,subsec:4:7:pertrope}). Hallucination Tendency is demonstrated by (1) LLMs' precision becomes much worse when CoT is equipped (Section \ref{subsec:4:4:cot,subsec:4:5:reasoningmode}), (2) Instances where CoT provides correct answers with wrong reasons (Section \ref{subsec:4:9:doublyright}), and (3) LLMs Injecting multiple trope-related text tokens without explicitly introducing a trope in a movie synopsis can lead to LLMs being misled by keywords and patterns (Section \ref{subsec:4:10:attack}).

%3.2 parallelly process concepts

%When significantly simplified TiMoS to binary classification task of each trope, GPT-4 can somehow perform reasoning on TiMoS dataset and barely surpass conventional supervised methods, which have less than 0.01\% parameters compared to it. However, the performance is still far behind humans. In addition, this suggests that LLMs cannot parallelly process multiple concepts and perform reasoning at once as humans do \cite{Huang2011}. 
%Further analysis discovers LLMs' limitations and highlights findings as follows: (1) While chain-of-thoughts prompting significantly improves the recall, it trades the precision off by conceiving and hallucinating based on information provided in movie synopses, which could be an issue in building trustworthy applications. (2) LLMs excel at capturing surface signals instead of comprehending across plots, resulting in performance improvement on several depictable tropes, but performance drops on tropes that require complex reasoning across different plots. (3) When injecting several trope related text tokens without bringing a trope to a movie synopsis, LLMs can be easily fooled by these keywords and patterns. This highlights previously mentioned issues of over-relying on surface signals and raises the security concern of the development of applications. (4) Even chain-of-thought boosts the performance, we observe various cases where LLMs do not reason ``doubly right'': The prediction is correct but the reason is wrong. This again highlights the trustworthy issues and the over reliance of surface signals.

%By comprehensively analyzing the results,  we also find two limitations of modern LLMs: (1) Even chain-of-thought improves the performance on binary-TiMoS, the thoughts are sometimes flawed when the answer is correct, indicating that LLMs do not truly understand. (2) LLM's prediction can be changed by injecting several keywords without modifying the synopses, revealing the reliance of certain patterns as if traditional supervised learning models.
%Upon further analysis, we have identified limitations in LLMs and present the following key findings: (1) Although CoT prompting significantly enhances recall, it does so at the expense of precision, as it may lead to the hallucination of content based on information from movie synopses. This trade-off could pose challenges in developing trustworthy applications. 
%(2) LLMs excel in capturing \revise{shallow semantic which could be identified with a single scene from a plot, }
%surface-level signals 
%but struggle with comprehensive understanding across different plot elements. While they perform well on certain recognizable tropes, their performance declines on tropes requiring complex reasoning spanning multiple plot points. 
%(3) Injecting multiple trope-related text tokens without explicitly introducing a trope in a movie synopsis can lead to LLMs being misled by keywords and patterns. This highlights concerns related to the overreliance on shallow semantics and raises security issues in application development. 
%(4) Despite the performance boost from CoT prompting, instances arise where LLMs provide correct predictions with incorrect reasoning. This once again underscores trustworthiness issues and the overdependence on shallow semantics. %\xudong{surface-level signals are mentioned multiple times here but I am a bit concerned whether we have very good quantitative results to demonstrate why the current signals leveraged is surface-level. additionally, it will be easier for the audience to refer to if the reference to sections can be also added here}

==> tables/exp_old.tex <==

\begin{table}[ht]
\centering
\begin{tabular}{lccc}
% {p{2.8cm}p{1cm}p{1.2cm}p{1cm}}
\toprule[1pt]
\textbf{Models} & F1&  P \tablefootnote{Baselines reported by TiMoS \cite{chang2021situationtimos} (first block) employs mean average precision(mAP) across various thresholds, while our approach (other blocks) directly predicts the answer and opts for Precision.} & R \\
% && Precision\\
%. Our approach, however, focuses on direct answer prediction and opts for Precision, utilizing a singular threshold.} 
\hline
  Random & 13.97 & 8.14 &-  \\
 BERT(fine-tuned) & 23.97 & 17.26 &- \\
MulCom & 25.00 & 18.73 & -\\ 
Human & 64.87 & 65.77 & 63.98 \\
\hline
\textbf{LLM Fine-Tuned} \\
Llama \\
\hline
 \textbf{LLM Prompt }  \\
\underline{\textbf{Base}} \\
% \hline
 Llama & 15.42 & 8.52 & \textbf{97.22}\\
 ChatGPT  & 18.06 &  20.81 &  22.10   \\ 
 GPT-4& \textbf{26.18} & \textbf{24.45} & 43.49 \\
 \underline{\textbf{Chain of Thought}} &  \\
  % \hline
  ChatGPT  & 21.11 & 14.08 & 70.16 \\
\bottomrule [1pt]
\end{tabular}
% \vspace{-0.3cm}
\caption{
%TiMoS \cite{chang2021situationtimos} sets the baseline with its supervised learning model, employing mean average precision(mAP) across various thresholds. Our approach, however, focuses on direct answer prediction and opts for Precision, utilizing a singular threshold. The battlefield is then divided: the second block showcases scores for the multi-label task, while the third drills down into the binary trenches, separating the Base and CoT prompt strategies.
%First block obtained from \cite{chang2021situationtimos}. Second block shows that LLMs only reach random guess-level performance on TiMoS dataset (Section\ref{subsec:4:2:mainresults}). Third block shows results in simplified binary classification task (Figure \ref{fig:figure2} and Section \ref{subsec:4:3:binaryresults})
The first block is extracted from \cite{chang2021situationtimos}. The second block shows that LLMs achieve performance equivalent to random guessing on the TiMoS dataset, as discussed in Section \ref{subsec:4:2:mainresults}. The third block presents the results of a simplified binary classification task, as shown in Figure \ref{fig:overview} and detailed in Section \ref{subsec:4:3:binaryresults}.
}
\label{table:2}
% \vspace{-0.3cm}
\end{table}



% The supervised learning model in the baseline, obtained from TiMoS\cite{chang2021situationtimos}, employs mean average precision(mAP) with varying thresholds. In contrast, our method focuses on direct answer prediction and opts for Precision, utilizing a singular threshold. The second block represents scores for Multi-label task, while the third block dissects results into Binary tasks, discerning between scores for Base and CoT Prompt methodologies



==> tables/motivation.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{ll|ccc|cc}
       Benchmark  & Task & LLM & SL & Human & $\delta$ SL & $\delta$ Human \\
       \hline
       SuperGLUE \cite{wang2019superglue}  & NLU & 91.2 & 71.5 & 89.8 & +19.7 & +1.4\\ 
       CommonSenseQA \cite{talmor2019commonsenseqa} & CS & 84.0 & 56.0 & 89.0 & +28.0 & -5.0 \\
       RadNLI \cite{miura-etal-2021-improving} & Medical & 89.3 & 79.8 & - & +9.5 & -\\
       GSM8K \cite{cobbe2021traininggsm8k} & Math & 57.0 & 55.0 & - & +2.0 & - \\
       LogiQA 2.0 \cite{liu2023logiqa} & %Logic & 72.25 & 48.76 & 86.00 & 23.47 & -13.75 \\
       Logic & 72.3 & 48.8 & 86.0 & +23.5 & -13.7 \\
       \hline
       %TiMoS \cite{chang2021situationtimos} & Trope & 8.77 & 25.00 & 64.00 & \textbf{-16.23} & \textbf{-55.23} \\
       TiMoS \cite{chang2021situationtimos} & Trope & 8.8 & 25.0 & 64.0 & \textbf{-16.23} & \textbf{-55.23} \\
    \end{tabular}
    \caption{
    \textbf{LLMs struggle to tackle the tropes in movie synopses (TiMoS) task despite dominating various NLP tasks. }\tablefootnote{SuperGLUE and CommonSenseQA performance obtained from \cite{singh2023mindscores1}, RadNLI from \cite{miura-etal-2021-improving}, GSM8K from \cite{wei2022chaincot}, LogiQA from \cite{liu2023evaluating}} 
    %SuperGLUE and CommonSenseQA performance obtained from \cite{singh2023mindscores1}, RadNLI from \cite{miura-etal-2021-improving}, GSM8K
    }
    \label{tab:motivation}
\end{table*}
